Variable Inertia Model Predictive Control for Fast Bipedal Maneuvers

This paper proposes a novel control framework for agile and robust bipedal locomotion, addressing model discrepancies between full-body and reduced-order models. Specifically, assumptions such as constant centroidal inertia have introduced significant challenges and limitations in locomotion tasks. To enhance the agility and versatility of full-body humanoid robots, we formalize a Model Predictive Control (MPC) problem that accounts for the variable centroidal inertia of humanoid robots within a convex optimization framework, ensuring computational efficiency for real-time operations. In the proposed formulation, we incorporate a centroidal inertia network designed to predict the variable centroidal inertia over the MPC horizon, taking into account the swing foot trajectories -- an aspect often overlooked in ROM-based MPC frameworks. By integrating the MPC-based contact wrench planning with our low-level whole-body controller, we significantly improve the locomotion performance, achieving stable walking at higher velocities that are not attainable with the baseline method. The effectiveness of our proposed framework is validated through high-fidelity simulations using our full-body bipedal humanoid robot DRACO 3, demonstrating dynamic behaviors.

==> sections/problem_statement_locomanipulation.tex <==
%   *start with a key diagram 
%%%%%%
%   * 1) what is novel compared to SOTA?
%-- In comparison to the single rigid body model based MPC, which assumes constant inertia over the prediction horizon, the proposed MPC framework considers the composite rigid body inertia variations over the prediction horizon to reduce the discrepancy between the models for planning and control by incorporating whole-body kinematics of a robot. In turn, this enables planning whole-body orientation (WBO) task trajectories for more agile and natural motions. In specific, states advantages of modelling inertia~~. A. Inertia modelling from offline learning -> reduce computation time (skip IK) B. considering swing Leg trajectory -> incorporate leg kinematics and roll-out inertia over the horizon C. planning WBO trajectories D. the robots with non-negligible distal mass -> significant inertia variation while swinging legs E. Convex formulation -> real-time computation available F. reduce model discrepancy between the planning and control.
%   * 2) how it broadly applies to many engineering settings?
%   * 3) what technical parts make it challenging to solve?

\subsection{Preliminaries}


\subsection{Problem Statement}
Recent works address the legged locomanipulation problem using MPC-based controllers~\cite{Sleiman2021AManipulation, Li2023Kinodynamics-basedLoco-manipulation}, but they mostly rely on footstep strategies that are external to the optimization, which often results in kinematic reachability issues. Although there are MPC-based locomotion frameworks~\cite{Bledt2017Policy-regularizedCheetah, Romualdi2022OnlineAdjustment} that optimize the reduced-order dynamic model along with footsteps, they rely on nonlinear programming that is prone to local minima and relatively low control frequency, posing challenges for real-time control performance.  

We tackle the problem of loco-manipulation for humanoid robots equipped with two arms. To this end, we propose a unified locomanipulation framework that optimizes reduced-order robot dynamic and object dynamic model along with the footstep, taking into account the multi-body centroidal angular momentum (CAM).    

%1. Given model (simplified model <-> full-order model)
% 2. Unknown object properties -> mass/inertia
% -> why is this important? -> when two objects have the same mass but different inertia.
% -> the inertia is a function of state (end-effector's orientation)
% -> if we consider the objects as disturbances, it is difficult to formalize the effect of the inertia when handling the objects
% -> we may lose the balance while handling the object due to non-considered inertia effects.
% 3. Model discrepancy
% -> reduced-order model (linear only) vs. reduced-order model (linear + angular)
% -> locomotion planning with external disturbance (function of the state)
% 4. Whole-body control
% -> improve the structure considering the state-dependent disturbance

% =========================================
% 1. mass (isometric inertia  vs. non-isometric inertia)
% 2. task tracking and balance issues

% =========================================
% **\textbf{trajectory opt / contact-posture opt}**\\
% 1. What is the best object manipulation posture for robots?
% 2. What is the optimal contact location with respect to the object CoM (or additionally reference manipulation force, if applicable)?\\
% **\textbf{locomanipulation mpc layer}** \\
% 1. How to handle object dynamics?
% \begin{itemize}
%     \item Augment object states with simplified robot model (++ explicit coupling with object-robot -- computational expansiveness)
%     \item Treated as an external force/moment (++ computational advantages -- non unified control framework for robot-object and thus unable to exploit the object for balancing) 
% \end{itemize} 
% 2. What control model?
% \begin{itemize}
%     \item reduced order model (++ computationally tractable and thus applicable to real-time control -- unmodelled arm and leg dynamics and thus rely on hand-crafted task trajectory)
%     \item full-order model (++ reflect precise dynamic model -- computational expansiveness)
% \end{itemize}
% 3. How to handle the model discrepancy (between the reduced and full order model)?
% \begin{itemize}
%     \item adaptive control for residual dynamics
%     \item learning approach for residual dynamics
% \end{itemize}





% The equation of motion in \eqref{eq:linear} is linear in terms of $\mathbf{p}_c$, $\mathbf{r}_{i}$, $\mathbf{f}_{i}$, $\bm{\tau}_{i}$ for all $i \in \{1, \cdots, n \}$. However,
% Note that Eq.~\eqref{eq:angular} is nonlinear because of the cross-product term and does not explicitly contain both the orientation and inertia states, while Eq.~\eqref{eq:linear} does have one (position and mass). The above dynamics model can be rewritten by newly introducing a state variable $\bm{x}=[\bm{p}_c^{\top}, ^{\mathcal{I}}\mathbf{R}_{\mathcal{B}}^{\top}, \dot{\bm{p}}_c^{\top}, ^{\mathcal{B}}\bm{w}^{\top}]^{\top} \in \mathbb{R}^{n_x}$ where $^{\mathcal{I}}\mathbf{R}_{\mathcal{B}} \in SO(3)$ and $^{\mathcal{B}}\bm{w}$ denote the orientation of the body frame $\mathcal{B}$ with respect to the inertial frame $\mathcal{I}$ and the angular velocity of the body, respectively:
% \begin{align*}
%     \dot{\bm{x}} = \bm{f}(\bm{x}, \bm{u}) = 
%     \begin{Bmatrix} 
%     \dot{\bm{p}}_c \\     
%     ^{\mathcal{I}}\dot{\mathbf{R}}_{\mathcal{B}} \\
%     \ddot{\bm{p}}_c \\
%     ^{\mathcal{B}}\dot{\bm{w}}
%     \end{Bmatrix} = 
%     \begin{Bmatrix}
%         \dot{\bm{p}}_c \\
%         ^{\mathcal{I}}\mathbf{R}_{\mathcal{B}}[^{\mathcal{B}}\bm{w}]_{\times} \\
%         \frac{1}{m}\sum_{i=1}^{n} \mathbf{f}_i + \mathbf{g} \\
%         ^{\mathcal{B}}\mathbf{I}^{-1}(^{\mathcal{B}}\bm{\tau} -^{\mathcal{B}}\bm{w} \times ^{\mathcal{B}}\mathbf{I}^{\mathcal{B}}\bm{w}) 
%     \end{Bmatrix},
% \end{align*}
% \begin{equation} \label{eq:centroidal_state_space_model}
    % \dot{\bm{x}} = \bm{f}(\bm{x}, \bm{u}) = \left[ 
%     \begin{array}{c}
%         \dot{\bm{p}}_c \\
%         ^{\mathcal{I}}\mathbf{R}_{\mathcal{B}}[^{\mathcal{B}}\bm{w}]_{\times} \\
%         \frac{1}{m}\sum_{i=1}^{n} \mathbf{f}_i + \mathbf{g} \\
%         ^{\mathcal{B}}\mathbf{I}^{-1}(^{\mathcal{B}}\bm{\tau} -^{\mathcal{B}}\bm{w} \times ^{\mathcal{B}}\mathbf{I}^{\mathcal{B}}\bm{w}) 
%     \end{array} \right]
% \end{equation}
% where $[\mathbf{a}]_{\times} \in so(3)$ denotes the skew symmertic matrix spanned from a vector $\mathbf{a}\in \mathbb{R}^{3}$. $^{\mathcal{B}}\mathbf{I}$ and $^{\mathcal{B}}\bm{\tau}$ represent the inertia tensor in the body frame and the net moment about the CoM, respectively.   

% Through the above assumptions, we can simplify the rotational dynamics in \eqref{eq:centroidal_state_space_model} using Euler angle representation and the following state-space model is obtained:
% \begin{align}
%     \dot{\bm{x}} = \bm{f}(\bm{x}, \bm{u})= \left[ 
%     \begin{array}{c}
%         \dot{\bm{p}}_c \\
%         ^{\mathcal{B}}\bm{w} \\
%         \frac{1}{m}\sum_{i=1}^{n} \mathbf{\Phi}_i\mathbf{f}_i + \mathbf{g} \\
%         {^{\mathcal{B}}\mathbf{I}^{-1}} \sum_{i=1}^{n}(\mathbf{R}_z^T(\psi)[\bm{r}_i]_\times\mathbf{\Phi}_i\mathbf{f}_i + \mathbf{R}_z^T(\psi)\mathbf{\Phi}_i\mathbf{\bm{\tau}}_i)
%     \end{array}\right]
% \end{align}
% \begin{align}
%     \dot{\bm{x}} = \bm{f}(\bm{x}, \bm{u}) = 
%     \begin{Bmatrix} 
%     \dot{\bm{p}}_c \\     
%     \dot{\bm{\Theta}} \\
%     \ddot{\bm{p}}_c \\
%     ^{\mathcal{B}}\dot{\bm{w}}
%     \end{Bmatrix} = 
%     \begin{Bmatrix}
%         \dot{\bm{p}}_c \\
%         ^{\mathcal{B}}\bm{w} \\
%         \frac{1}{m}\sum_{i=1}^{n} \mathbf{\Phi}_i\mathbf{f}_i + \mathbf{g} \\
%         {^{\mathcal{B}}\mathbf{I}^{-1}} \sum_{i=1}^{n}(\mathbf{R}_z^T(\psi)[\bm{r}_i]_\times\mathbf{\Phi}_i\mathbf{f}_i)
%     \end{Bmatrix},
% \end{align}
% where $\bm{\Theta}$ denotes Euler angles as $\bm{\Theta}= [\theta, \phi, \psi]$ with an earth-fixed roll($\theta$), pitch($\phi$), yaw($\psi$) convention and $\mathbf{\Phi}_i \in \{0, 1\}$ represents the $i^{th}$ end-effector contact state at a given time instant. In addition, we specify the state $\bm{x} = [\bm{p}_c^{\top}, \bm{\Theta}^{\top}, \dot{\bm{p}}_c^{\top}, ^{\mathcal{B}}\bm{w}^{\top}]^{\top} \in \mathbb{R}^{n_x}$ and control input $\bm{u} = [\bm{f}_1^{\top}, \bm{\tau}_1^{\top} \cdots \bm{f}_n^{\top}, \bm{\tau}_n^{\top}]^{\top}\in\mathbb{R}^{n_u}$ in the above state-space model. 
% The discrete dynamics are given as
% \begin{align*}
%     \bm{x}_{k+1} = \mathbf{A}_k\bm{x}_k + \mathbf{B}_k(\overline{\mathbf{I}}_k)\bm{h}(\bm{x}_k, \bm{u}_k, \bm{\Phi}_k) + \bm{d}_k,
% \end{align*}
% where $\mathbf{A}_k$, $\mathbf{B}_k$, and $\bm{d}_k$ are written as
% \begin{align*}
%         \mathbf{A}_k = \begin{bmatrix}
%             \mathbf{I}_{6\times6} & \Delta t_k\mathbf{I}_{6\times6} \\
%             \bm{0}_{6\times6} & \mathbf{I}_{6\times6}
%         \end{bmatrix},
%         & \mathbf{B}_k = \begin{bmatrix}
%             \frac{\Delta t_k^2}{2}\ ^{\mathcal{B}}\overline{\mathbf{I}}_k^{-1}  \\
%             \Delta t_k \ ^{\mathcal{B}}\overline{\mathbf{I}}_k^{-1}
%         \end{bmatrix}, \\
%         \bm{h}(\bm{x}_k, \bm{u}_k, \bm{\Phi}_k) = \sum_{i=1}^{n_{ee}}\begin{bmatrix}
%             \mathbf{I}_{3\times3} 
%             \mathbf{R}_z^T(\psi_k)[\bm{r}_{i,k}]_\times
%         \end{bmatrix}\mathbf{\Phi}_{i,k}\mathbf{f}_{i,k},
%         & \bm{d}_k = \begin{bmatrix}
%             \frac{\Delta t_k^2}{2} \bm{a}_g  \\
%             \Delta t_k \bm{a}_g
%         \end{bmatrix},
% \end{align*}
% with $^{\mathcal{B}}\overline{\mathbf{I}}_k^{-1} = \textrm{diag}(\frac{1}{m}\mathbf{I}^{-1}_{3\times3}, ^{\mathcal{B}}\mathbf{I}_k^{-1})$ and $\bm{a}_g = [\bm{g}^T, \bm{0}_{3\times1}^T]^T$. For simplicity, we use forward Euler integration to approximate the time derivative function for velocities while trapezoidal integration is used for position quantities.
